Dynamic Minimum Spanning Forest with Subpolynomial Worst-case Update Time

We present a Las Vegas algorithm for dynamically maintaining a minimum spanning forest of an $n$-node graph undergoing edge insertions and deletions. Our algorithm guarantees an $O(n^{o(1)})$ worst-case update time with high probability. This significantly improves the two recent Las Vegas algorithms by Wulff-Nilsen [STOC'17] with update time $O(n^{0.5-\epsilon})$ for some constant $\epsilon>0$ and, independently, by Nanongkai and Saranurak [STOC'17] with update time $O(n^{0.494})$ (the latter works only for maintaining a spanning forest). Our result is obtained by identifying the common framework that both two previous algorithms rely on, and then improve and combine the ideas from both works. There are two main algorithmic components of the framework that are newly improved and critical for obtaining our result. First, we improve the update time from $O(n^{0.5-\epsilon})$ in Wulff-Nilsen [STOC'17] to $O(n^{o(1)})$ for decrementally removing all low-conductance cuts in an expander undergoing edge deletions. Second, by revisiting the "contraction technique" by Henzinger and King [1997] and Holm et al. [STOC'98], we show a new approach for maintaining a minimum spanning forest in connected graphs with very few (at most $(1+o(1))n$) edges. This significantly improves the previous approach in [Wulff-Nilsen STOC'17] and [Nanongkai and Saranurak STOC'17] which is based on Frederickson's 2-dimensional topology tree and illustrates a new application to this old technique.

==> improved_flow.tex <==

\section{Improved Local Flow Algorithms\label{sec:improved flow}}

For a detailed proof, we first note the following fact which holds
simply because flows and preflows preserve the overall supply. 
\begin{fact}
For any preflow $f$ with source function $\Delta$, $\sum_{v}f(v)=\sum_{v}\Delta(v)+\sum_{v,u}f(u,v)=\total{\Delta}$.
Consequently, $\total{ex}+\total{ab}=\total{\Delta}$\label{fact:total supply}

\danupon{Can we cite other papers for the above fact? Do we need to give a short proof?}\danupon{TO DO: We should seperate the fact above into 2-3 equalities so readers know which one(s) we use at each point.}
\end{fact}

\subsection{Excess Scaling Flow}

In this section, we apply excess scaling technique from \cite{HenzingerRW17}
to \ref{thm:mod Unit Flow} in the exactly same way as when it is
applied to \ref{thm:orig unit flow} in \cite{HenzingerRW17}. The
important property of this algorithm is that it lower bounds the volume
of the outputted cut.
\begin{lem}
\label{lem:excess scaling flow}Given a graph $G=(V,E)$ with $m$
edges (with parallel edges but no self loop and isolated node), a
parameter $F$, a source function $\Delta$ such that $\Delta(v)\le F\cdot\deg(v)$
for all $v\in V$, a sink function $T$ where $T(v)\le\deg(v)$ for
all $v\in V$ and $\total{\Delta}\le\total T$, a constant $0<\tau<1$,
and positive parameters $U$ and $h\ge\log m$, Excess Scaling Flow
algorithm will, in time $O(h(\total{\Delta}+\total{\overline{T}}\log m))$,
return one of the following two cases:
\begin{enumerate}
\item A preflow flow $f$ for $(G(UF),\Delta,T)$ where $\total{ex_{f}}\le\tau\total{\Delta}$.
\item A cut $S$ where $\phi(S)\le\frac{20\log2m}{h}+\frac{4}{U}$ and $vol(S)=\Omega(\frac{\tau\total{\Delta}}{F\log m}).$
\end{enumerate}
\end{lem}
This theorem can be proved in almost the same way as \cite[Lemma 3.2]{HenzingerRW17}
but our proof is a bit more complicated.\footnote{\ref{alg:Excess Scaling} is somewhat different from \cite[Algorithm 3.2]{HenzingerRW17}
because 1) in Step 5 we have the condition $\forall v:\Delta_{j+1}(v)\le T(v)$
instead of $\forall v:\Delta_{j+1}(v)\le\deg(v)$ because maybe $T(v)<\deg(v)$
for some $v$ in our setting, and 2) the change in Step 3 and other
changes are mainly for enforcing the preflow and source functions
to be integral. (In \cite{HenzingerRW17}, they also need source functions
to be integral, it is not clear for us how to this follows directly
from their algorithm.) To make everything being integral, this makes
an argument more complicated.} We include it here for completeness. See \ref{alg:Excess Scaling}
for the description of the algorithm.

In Step 1, we run Unit Flow algorithm from \ref{thm:mod Unit Flow}
where the parameter $w$ for Unit Flow algorithm is always set to
be $w=4$. For a function $\Delta_{j}$ and a number $\mu_{j}$, we
denote $\left\lfloor \frac{\Delta_{j}(\cdot)}{\mu_{j}}\right\rfloor $
as a function which outputs $\left\lfloor \frac{\Delta_{j}(v)}{\mu_{j}}\right\rfloor $
for each $v$. After running $UnitFlow(G,w=4,\left\lfloor \frac{\Delta_{j}(\cdot)}{\mu_{j}}\right\rfloor ,T,U,h)$,
Unit Flow algorithm returns a preflow $f_{j}$ for $(G(U,\left\lfloor \frac{\Delta_{j}(\cdot)}{\mu_{j}}\right\rfloor ,T)$
and possibly a cut $A_{j}$. By \ref{rem:output flow}, we also obtained
the excess and absorb functions $ex_{j}$ and $ab_{j}$ w.r.t. $f_{j}$,
$\left\lfloor \frac{\Delta_{j}(\cdot)}{\mu_{j}}\right\rfloor $ and
$T$.

\begin{algorithm}[H]
\caption{\label{alg:Excess Scaling} $ExcessScalingFlow(G,F,\Delta,T,\tau,U,h)$}

\begin{description}
\item [{Initialization:}]~


Let $\mu_{0}=2^{k}$ for some $k$ where $F/4\le\mu_{0}<F/2$. 


Let $\mu_{i}=\mu_{0}/2^{i}$ for any $i$. 


Let $\Delta_{0}=\Delta$, $j=0$, and $f$ be a zero preflow.

\item [{Repeat}]~

\begin{enumerate}
\item Run $UnitFlow(G,w=4,\left\lfloor \frac{\Delta_{j}(\cdot)}{\mu_{j}}\right\rfloor ,T,U,h)$
and get back $f_{j}$ (in unit $\mu_{j}$), $ab_{j}$ and $A_{j}$.
\item Add $f_{j}$ in unit $\mu_{j}$ to our current preflow: $\forall(v,u)$
$f(v,u)\gets f(v,u)+f_{j}(v,u)\mu_{j}$.
\item Set a new source function $\Delta_{j+1}$: $\forall v$ 
\[
\Delta_{j+1}(v)=ab_{j}(v)\mu_{j}+\Delta_{j}(v)\bmod\mu_{j}.
\]

\item \textbf{If }$vol(A_{j})\ge\frac{\tau\total{\Delta}}{4\mu_{j}\log m}$,
\textbf{Return} cut $S=A_{j}$ (case 2).
\item \textbf{If }$\forall v:\Delta_{j+1}(v)\le T(v)$, \textbf{Return}
preflow $f$ (case 1).
\item $j\gets j+1$.
\end{enumerate}
\item [{End}] \textbf{Repeat}\end{description}
\end{algorithm}


The rest of this section is for the proof of \ref{lem:excess scaling flow}.
First, we show that the input $(G,w=4,\left\lfloor \frac{\Delta_{j}(\cdot)}{\mu_{j}}\right\rfloor ,T,U,h)$
is a valid input for Unit Flow algorithm.
\begin{lem}
For all $j$ and $v$, $\left\lfloor \Delta_{j}(v)/\mu_{j}\right\rfloor \le4\deg(v)$.\end{lem}
\begin{proof}
For $j=0$, we have $\left\lfloor \frac{\Delta(v)}{\mu_{0}}\right\rfloor \le\left\lfloor \frac{F\deg(v)}{F/4}\right\rfloor =4\deg(v)$
for all $v\in V$ because $F/4\le\mu_{0}$. For $j>0$, we have 
\begin{eqnarray*}
\left\lfloor \Delta_{j}(v)/\mu_{j}\right\rfloor  & \le & \frac{ab_{j-1}(v)\mu_{j-1}+\Delta_{j-1}(v)\bmod\mu_{j-1}}{\mu_{j}}\\
 & \le & \frac{T(v)\mu_{j-1}+\mu_{j-1}}{\mu_{j}}\\
 & \le & 2\deg(v)+2\le4\deg(v),
\end{eqnarray*}
where the last inequality is because there is no isolated nodes.
\end{proof}
Next, we show the termination and running time.
\begin{lem}
\ref{alg:Excess Scaling} must terminate when $j=k\le\log m$ and
the total running time is $O(h(\total{\Delta}+\total{\overline{T}}\log m))$.\label{thm:excess scaling time}\end{lem}
\begin{proof}
When $j=k$, we have $\mu_{j}=1$. In Step 3, we set $\Delta_{j+1}(v)=ab_{j}(v)\le T(v)$
for all $v$, which satisfies the condition of Step 5.

At the iteration $j$, Unit Flow algorithm takes $O(wh(\left\lfloor \Delta_{j}(\cdot)/\mu_{j}\right\rfloor +\total{\overline{T}}))$
time and this dominates the time for other steps. In total, the running
time is $\sum_{j\le\log m}O(wh(\left\lfloor \Delta_{j}(\cdot)/\mu_{j}\right\rfloor +\total{\overline{T}}))=O(h(\total{\Delta}+\total{\overline{T}}\log m))$.
Note that $w=4$ is a constant.
\end{proof}
Suppose that \ref{alg:Excess Scaling} terminates when $j=j^{*}\le k$,
by \ref{thm:excess scaling time}. Now, we show the correctness of
the output of the algorithm.
\begin{lem}
If \ref{alg:Excess Scaling} terminates with Step 4, then $\phi(S)\le\frac{20\log2m}{h}+\frac{4}{U}$
and $vol(S)=\Omega(\frac{\tau\total{\Delta}}{F\log m})$.\label{thm:excess scaling cut correct}\end{lem}
\begin{proof}
We have $\phi(S)\le\frac{20\log2m}{h}+\frac{4}{U}$ by \ref{thm:mod Unit Flow}.
As the algorithms terminates in Step 4, we have that $vol(S)\ge\frac{\tau\total{\Delta}}{4\mu_{j^{*}}\log m}=\Omega(\frac{\tau\total{\Delta}}{F\log m})$
because $\mu_{j^{*}}\le\mu_{0}\le F/2$.
\end{proof}
It it left to show the correctness when \ref{alg:Excess Scaling}
terminates with Step 5. To do this, we need two claims which crucially
rely on the choice of the definition of $\Delta_{j+1}$ in Step 3
of \ref{alg:Excess Scaling}.
\begin{claim}
After termination, a preflow $f$ is source-feasible w.r.t. $\Delta$.\label{thm:source-feasible}\end{claim}
\begin{proof}
We need to show that $f$ is also source-feasible w.r.t. $\Delta$,
i.e. $\sum_{u}f(u,v)\le\Delta(v)$ for all $v\in V$: 

\begin{eqnarray*}
\sum_{u}f(u,v) & = & \sum_{j\le j^{*}}\sum_{u}f_{j}(u,v)\mu_{j}\\
 & = & \sum_{j\le j^{*}}\left\lfloor \frac{\Delta_{j}(v)}{\mu_{j}}\right\rfloor \mu_{j}-f_{j}(v)\mu_{j}\\
 & = & \left\lfloor \frac{\Delta_{0}(v)}{\mu_{0}}\right\rfloor \mu_{0}+(\sum_{j<j^{*}}\left\lfloor \frac{\Delta_{j+1}(v)}{\mu_{j+1}}\right\rfloor \mu_{j+1}-f_{j}(v)\mu_{j})-f_{j^{*}}(v)\mu_{j^{*}}\\
 & \le & \left\lfloor \frac{\Delta_{0}(v)}{\mu_{0}}\right\rfloor \mu_{0}+\Delta_{0}(v)\bmod\mu_{0}-\Delta_{j+1}(v)\bmod\mu_{j+1}-f_{j^{*}}(v)\mu_{j^{*}}\\
 & \le & \Delta_{0}(v)=\Delta(v),
\end{eqnarray*}
where the first inequality is because $\left\lfloor \frac{\Delta_{j+1}(v)}{\mu_{j+1}}\right\rfloor \mu_{j+1}-f_{j}(v)\mu_{j}\le\Delta_{j}(v)\bmod\mu_{j}-\Delta_{j+1}(v)\bmod\mu_{j+1}$,
which is true because of the definition of $\Delta_{j+1}$: 
\begin{eqnarray*}
\left\lfloor \frac{\Delta_{j+1}(v)}{\mu_{j+1}}\right\rfloor \mu_{j+1}+\Delta_{j+1}(v)\bmod\mu_{j+1} & = & \Delta_{j+1}(v)\\
 & = & ab_{j}(v)\mu_{j}+\Delta_{j}(v)\bmod\mu_{j}\\
 & \le & f_{j}(v)\mu_{j}+\Delta_{j}(v)\bmod\mu_{j}.
\end{eqnarray*}
\end{proof}
\begin{claim}
After termination with Step 5, $\total{ex_{f}}=\sum_{j\le j^{*}}\total{ex_{j}}\mu_{j}$.\label{thm:total excess}\end{claim}
\begin{proof}
Note that $f_{j}$ is a preflow with source function $\left\lfloor \Delta_{j}(\cdot)/\mu_{j}\right\rfloor $.
So $\sum_{v}f_{j}(v)=\left\lfloor \Delta_{j}(\cdot)/\mu_{j}\right\rfloor $
by \ref{fact:total supply}. By the definition of $\Delta_{j+1}$
and because $ab_{j}(v)=f_{j}(v)-ex_{j}(v)$, we have 
\[
\Delta_{j}(v)\bmod\mu_{j}+f_{j}(v)\mu_{j}=\Delta_{j+1}(v)+ex_{j}(v)\mu_{j}
\]
 for any $j,v$. Summing over all nodes $v$, we have on one hand
\begin{eqnarray*}
\sum_{v}(\Delta_{j}(v)\bmod\mu_{j}+f_{j}(v)\mu_{j}) & = & \sum_{v}(\Delta_{j}(v)\bmod\mu_{j}+\left\lfloor \Delta_{j}(v)/\mu_{j}\right\rfloor \mu_{j})\\
 & = & \sum_{v}\Delta_{j}(v)=\total{\Delta_{j}}.
\end{eqnarray*}
On the other hand, 
\[
\sum_{v}\Delta_{j+1}(v)+ex_{j}(v)\mu_{j}=\total{\Delta_{j+1}}+\total{ex_{j}}\mu_{j}.
\]
So we have that 
\[
\sum_{j\le j^{*}}\total{ex_{j}}\mu_{j}=\sum_{j\le j^{*}}\total{\Delta_{j}}-\total{\Delta_{j+1}}=\total{\Delta_{0}}-\total{\Delta_{j^{*}+1}}.
\]
Since the algorithm terminates with Step 5, $\forall v:\Delta_{j+1}(v)\le T(v)$.
That is, $\total{\Delta_{j^{*}+1}}=\total{ab_{f}}$ is the total supply
absorbed by sinks. As $\Delta=\Delta_{0}$, we have by \ref{fact:total supply}
\[
\total{\Delta_{0}}-\total{\Delta_{j^{*}+1}}=\total{\Delta}-\total{ab_{f}}=\total{ex_{f}}.
\]
Therefore, we have $\total{ex_{f}}=\total{\Delta_{0}}-\total{\Delta_{j^{*}+1}}=\sum_{j\le j^{*}}\total{ex_{j}}\mu_{j}$.\end{proof}
\begin{lem}
If \ref{alg:Excess Scaling} terminates with Step 5, $f$ is a feasible
preflow for $(G(UF),\Delta,T)$ and the excess function $ex_{f}$
is such that $\total{ex_{f}}\le\tau\total{\Delta}$.\label{thm:excess scaling flow correct}\end{lem}
\begin{proof}
First, $f$ is capacity-feasible because by Step 2, for all $u,v$,
we have 
\[
|f(v,u)|\le\sum_{j\le j^{*}}|f_{j}(v,u)|\mu_{j}\le\sum_{j\le j^{*}}U\mu_{j}\le U\sum_{j\le j^{*}}F/2^{j+1}\le UF.
\]
Since $f$ is also source-feasible by \ref{thm:source-feasible},
$f$ is a feasible preflow. 

By \ref{thm:total excess}, $\total{ex_{f}}=\sum_{j\le j^{*}}\total{ex_{j}}\mu_{j}$.
For any cut $S'$, let $ex_{j}(S')=\sum_{v\in S}ex_{j}(v)$. We conclude
that

\[
\total{ex_{f}}=\sum_{j\le j^{*}}\total{ex_{j}}\mu_{j}\le\sum_{j\le j^{*}}ex_{j}(A_{j})\mu_{j}\le\sum_{j\le j^{*}}4vol(A_{j})\mu_{j}\le\sum_{j\le j^{*}}\frac{\tau\total{\Delta}}{\log m}\le\tau\total{\Delta}.
\]
The first two inequalities are by \ref{thm:mod Unit Flow}, which
says $ex_{j}(v)\le4\deg(v)$ if $v\in A_{j}$ and $ex_{j}(v)=0$ otherwise.
The last two inequalities are because $vol(A_{j})\le\frac{\tau\total{\Delta}}{4\mu_{j}\log m}$
for all $j\le j^{*}\le\log m$, because the condition in Step 4 is
never satisfied. 
\end{proof}
By \ref{thm:excess scaling time}, \ref{thm:excess scaling cut correct},
and \ref{thm:excess scaling flow correct}, we conclude the correctness
of \ref{lem:excess scaling flow}.


\subsection{Almost Flow (Proof of \ref{thm:Extended Unit Flow})}

In this section, we use Excess Scaling Flow algorithm as a subroutine
and obtain Almost Flow algorithm from \ref{thm:Extended Unit Flow}.
The description of the algorithm in \ref{alg:Almost Flow}.

\begin{algorithm}[H]
\caption{\label{alg:Almost Flow} $AlmostFlow(G,F,\Delta,T,U,h)$}

\begin{description}
\item [{Initialization:}] Let $\Delta_{0}=\Delta$, $T_{0}=T$, $j=0$,
and $f$ be a zero flow.
\item [{While}] $\total{\Delta_{j}}>0$ 

\begin{enumerate}
\item Run $ExcessScalingFlow(G,F,\Delta_{j},T_{j},\tau=1/2,U,h)$, and either
get a preflow $f_{j}$ (together with $ex_{j}$ and $ab_{j}$) or
a cut $S_{j}$. 
\item \textbf{If }a preflow $f_{j}$ is returned, \textbf{Update:} 

\begin{enumerate}
\item $\forall v$, $\Delta_{j+1}=ex_{j}$,
\item $\forall v$, $T_{j+1}(v)=T_{j}(v)-ab_{j}(v)$,
\item $\forall(u,v)$, $f(u,v)=f(u,v)+f_{j}(u,v)$.
\end{enumerate}
\item \textbf{Else }a cut $S_{j}$ is returned, \textbf{Return} $S=S_{j}$
and $f$ as the output.
\item $j\gets j+1$.
\end{enumerate}
\item [{End}] \textbf{Repeat}\end{description}
\end{algorithm}


First, we analyze the running time.
\begin{lem}
For any $j$, $\total{\Delta_{j}}+\total{\overline{T}_{j}}=\total{\Delta}+\total{\overline{T}}$.\label{lem:total supply preserve}\end{lem}
\begin{proof}
We will prove that $\total{\Delta_{j}}+\total{\overline{T}_{j}}=\total{\Delta_{j+1}}+\total{\overline{T}_{j+1}}$
for any $j$. By Step 2.b, we have that $\total{ab_{j}}=\total{T_{j}}-\total{T_{j+1}}=\total{\overline{T}_{j+1}}-\total{\overline{T}_{j}}$.
The following completes the proof. 
\[
\total{\Delta_{j}}=\sum_{v}f_{j}(v)=\sum_{v}ab_{j}(v)+ex_{j}(v)=\total{ab_{j}}+\total{ex_{j}}=\total{\overline{T}_{j+1}}-\total{\overline{T}_{j}}+\total{\Delta_{j+1}}.
\]
\end{proof}
\begin{lem}
\label{thm:almost flow time}\ref{alg:Almost Flow} must terminate
once $j=\left\lceil \log\total{\Delta}\right\rceil $, and the total
running time is $O(h(\total{\Delta}+\total{\overline{T}})\log m\log\total{\Delta})$\end{lem}
\begin{proof}
If the algorithm does not terminate at the $j$-th iteration, we have
$\total{\Delta_{j+1}}=\total{ex_{j}}\le\tau\total{\Delta_{j}}$ by
the property of Excess Scaling Flow algorithm from \ref{lem:excess scaling flow}.
So $\total{\Delta_{\left\lceil \log\total{\Delta}\right\rceil +1}}<1$.
Since $\total{\Delta_{\left\lceil \log\total{\Delta}\right\rceil +1}}$
is integral, $\total{\Delta_{\left\lceil \log\total{\Delta}\right\rceil }}=0$
and hence \ref{alg:Almost Flow} must terminate.

In the $j$-th iteration, Excess Scaling Flow algorithm runs in time
$O(h(\total{\Delta_{j}}+\total{\overline{T}_{j}}\log m))$, which
dominates other steps. Since $\total{\Delta_{j}}+\total{\overline{T}_{j}}=\total{\Delta}+\total{\overline{T}}$
by \ref{lem:total supply preserve}, the total run time is at most
$O(h(\total{\Delta}+\total{\overline{T}})\log m\log\total{\Delta})$.
\end{proof}
Next, we prove the correctness. Suppose that the algorithm terminates
at the iteration when $j=j^{*}$. 
\begin{lem}
$ab_{f}(v)=\sum_{j<j^{*}}ab_{j}(v)$ for any $v\in V$\label{thm:total absorb}\end{lem}
\begin{proof}
For any function $g$ and $i$, we note $g_{<i}(v)=\sum_{j<i}g_{j}(v)$
and $g_{>i}(v)=\sum_{j>i}g_{j}(v)$. Fix any $v$. We want to prove
that $ab_{<j^{*}}(v)=\min\{f(v),T(v)\}=ab_{f}(v)$.

There are two observations. First, $f(v)=f_{<j^{*}}(v)$. Second,
$ab_{<j}(v)=T(v)-T_{j}(v)$ for any $j$, by telescoping the equation
$T_{j}(v)=T_{j-1}(v)-ab_{j-1}(v)$.

Let $k<j^{*}$ be the smallest number where $f_{k}(v)\ge T_{k}(v)$.
Hence, for any $j<k$, $ab_{j}(v)=f_{j}(v)$. In particular, $ab_{<k}(v)=f_{<k}(v)$.
There are two cases:

For the first case, if $k$ exists, then $ab_{k}(v)=T_{k}(v)$ and
$T_{j}(v)=0$ for any $j>k$. So $ab_{>k}(v)=0$. As $ab_{<k}(v)=f_{<k}(v)=T(v)-T_{k}(v)$,
we get $ab_{<j^{*}}(v)=ab_{k}(v)+ab_{<k}(v)=T(v)$ while $f(v)=f_{<j^{*}}(v)=f_{k}(v)+f_{<k}(v)\ge T(v)$.
That is, $ab_{<j^{*}}(v)=T(v)$ when $f(v)\ge T(v)$.

For the second case, if $k$ does not exist, then $ab_{<j^{*}}(v)=f_{<j^{*}}(v)=f(v)$.
However, $f(v)=ab_{<j^{*}}(v)=T(v)-T_{j^{*}}(v)\le T(v)$. That is,
$ab_{<j^{*}}(v)=f(v)$ when $f(v)\le T(v)$.

From both cases, we conclude $ab_{<j^{*}}(v)=\min\{f(v),T(v)\}=ab_{f}(v)$.\end{proof}
\begin{lem}
\label{thm:almost flow correct}Let $s=\total{\Delta_{j^{*}}}$. We
have the following:
\begin{enumerate}
\item The outputted preflow $f$ is feasible for $(G(UF\left\lceil \log\total{\Delta}\right\rceil ),\Delta,T)$
and $\total{ex_{f}}<s.$ 
\item The outputted cut $S$ is such that $\phi_{G}(S)\le\frac{20\log2m}{h}+\frac{4}{U}\mbox{ and }vol(S)=\Omega(\frac{s}{F\log m}).$
\end{enumerate}
\end{lem}
\begin{proof}
First, $f$ is capacity-feasible because, for all $u,v,$ $|f(u,v)|\le\sum_{j\le j^{*}}|f_{j}(u,v)|\le UF\left\lceil \log\total{\Delta}\right\rceil $
where the last inequality is because $|f_{j}(u,v)|\le UF$ by \ref{lem:excess scaling flow}
and $j^{*}\le\left\lceil \log\total{\Delta}\right\rceil $ by \ref{thm:almost flow time}.

Next, $f$ is source-feasible w.r.t. $\Delta$ because, $\Delta_{j+1}(v)=ex_{j}(v)$
for all $v\in V$, that is the source supply at $v$ is just the excess
supply from previous iteration. So all supply being routed are ``from''
the source in the beginning. More formally, we have that, for all
$v$,
\begin{eqnarray*}
\sum_{u}f(v,u) & = & \sum_{j<j^{*}}\sum_{u}f_{j}(v,u)\\
 & = & \sum_{j<j^{*}}\Delta_{j}(v)-f_{j}(v)\\
 & = & \Delta_{0}(v)+(\sum_{j<j^{*}}\Delta_{j+1}(v)-f_{j}(v))-f_{j^{*}}(v)\\
 & = & \Delta_{0}(v)+(\sum_{j<j^{*}}ex_{j}(v)-f_{j}(v))-f_{j^{*}}(v)\le\Delta_{0}(v)
\end{eqnarray*}
where the last inequality is because $ex_{j}(v)\le f_{j}(v)$ by the
definitions. Therefore, $f$ is a feasible preflow for $(G(UF\left\lceil \log\total{\Delta}\right\rceil ),\Delta,T)$.

Next, we show that $\total{ex_{f}}=s$. By \ref{thm:total absorb},
we have
\begin{eqnarray*}
\total{ex_{f}} & = & \total{\Delta}-\total{ab_{f}}\\
 & = & \total{\Delta_{0}}-\sum_{j<j^{*}}\total{ab_{j}}\\
 & = & \total{\Delta_{0}}-(\sum_{j<j^{*}}\total{\Delta_{j}}-\total{ex_{j}})\\
 & = & \total{\Delta_{0}}-(\sum_{j<j^{*}}\total{\Delta_{j}}-\total{\Delta_{j+1}})\\
 & = & \total{\Delta_{j^{*}}}=s.
\end{eqnarray*}
This finishes the first part of the proof.

For the second part, we have that the cut $S$ is such that $\phi_{G}(S)\le\frac{20\log2m}{h}+\frac{4}{U}$
and $vol(S)=\Omega(\frac{\tau\total{\Delta_{j^{*}}}}{F\log m})=\Omega(\frac{s}{F\log m})$
just by \ref{lem:excess scaling flow} 
\end{proof}
By \ref{thm:almost flow time} and \ref{thm:almost flow correct},
we conclude the proof of \ref{thm:Extended Unit Flow}.

